Application of Facial Recognition using Convolutional Neural Networks for Entry Access Control

The purpose of this paper is to design a solution to the problem of facial recognition by use of convolutional neural networks, with the intention of applying the solution in a camera-based home-entry access control system. More specifically, the paper focuses on solving the supervised classification problem of taking images of people as input and classifying the person in the image as one of the authors or not. Two approaches are proposed: (1) building and training a neural network called WoodNet from scratch and (2) leveraging transfer learning by utilizing a network pre-trained on the ImageNet database and adapting it to this project's data and classes. In order to train the models to recognize the authors, a dataset containing more than 150 000 images has been created, balanced over the authors and others. Image extraction from videos and image augmentation techniques were instrumental for dataset creation. The results are two models classifying the individuals in the dataset with high accuracy, achieving over 99% accuracy on held-out test data. The pre-trained model fitted significantly faster than WoodNet, and seems to generalize better. However, these results come with a few caveats. Because of the way the dataset was compiled, as well as the high accuracy, one has reason to believe the models over-fitted to the data to some degree. An added consequence of the data compilation method is that the test dataset may not be sufficiently different from the training data, limiting its ability to validate generalization of the models. However, utilizing the models in a web-cam based system, classifying faces in real-time, shows promising results and indicates that the models generalized fairly well for at least some of the classes (see the accompanying video).

==> Sections/todos.tex <==
0 - Abstract
% Information box. TODO: remove before submitting
\todo[inline, color=lightgray!40]
{
    Welcome to the LaTeX template for the third assignment / main project report in TDT4173.
    To stay consistent (and save the author some time), it is based on the template used for Assignment 1 (which in turn was based on a template by Jon Arnt Kårstad, NTNU IMT), but you are free to choose any other template for your report as long as it roughly tracks the format laid out here \textbf{and does not exceed 10 pages} (excluding: title page, abstract, ToC, bibliography and appendices).
    
    \vspace{0.2cm}
    The page limits stated are for your orientation on how to structure your paper and are not hard limits.
}


\todo[inline, color=lightgray!40]
{
    In the abstract, give the reader an overview of the paper. Briefly, state the purpose of this project, what you did, as well as key findings and results. 
    
    \vspace{0.2cm}
    \textbf{Amount:} Up to 0.5 page 
}

1 - Introduction
\todo[inline, color=lightgray!40]
{
    Clearly state your problem and provide motivation for why it is interesting. This includes explicitly (but briefly) stating:
    \\\vspace{0.2cm}
    - Which task you are addressing in your project, e.g.: unsupervised clustering of typical daily price developments, supervised object detection of military bases, supervised prediction of total required cooking time, etc.
    \\\vspace{0.2cm}
    - What data you will be working with, e.g.: hourly electricity prices, aerial grayscale images, natural language cookie recipes, etc.
    \\\vspace{0.2cm}
    - Which method(s) you will use, e.g.: hierarchical agglomerative clustering, Faster R-CNN / deep learning, gradient boosted regression on term frequencies, etc.
    
    \vspace{0.2cm}
    \textbf{Amount:} 0.5 - 1 page
}



2 - Related work
\todo[inline, color=lightgray!40]
{
    Cite and briefly describe research that is related to the problem you are trying to solve (or problems that are highly analogous). Try to find a logical way to group them based on e.g. methodology or problem interpretation. You may also want to merge this section with the introduction if that feels more natural (use your own judgment).
    
    \vspace{0.2cm}
    It is common to use this part of a paper to show that you are familiar with the existing body of research and argue how your work contributes to it. However, since you are not required to do novel research in this project, it is sufficient to simply contextualize your project within the field.


    \vspace{0.2cm}
    \textbf{Amount:} 0.5 - 1 page
    
    Possible relevant related work:
    FaceNet:
    https://cmusatyalab.github.io/openface/
    https://arxiv.org/pdf/1503.03832.pdf
    
    
    Dropout against over-fitting:
    https://arxiv.org/abs/1207.0580
    
    
}

3 - Data
\todo[inline, color=lightgray!40]
{
    Describe your data, including where you sourced it from, its type, and dimensionality. The content in this section is highly dependent on your problem and how much preprocessing you'll have to do, but may include information such as:
    
    \vspace{0.2cm}
    - How you intend to split your data (train/test/valid) and how many samples there are in each split.
    
    \vspace{0.2cm}
    - Basic summary statistics of the data (mean, std, quantiles, etc) and visualizations. Prioritize the most salient content that may help you in rationalizing your choice of preprocessing and methods.
    
    \vspace{0.2cm}
    - Additional information on your preprocessing pipline, e.g. time-series featurization, feature filtering, PCA-transforms, word embeddings, normalization, image augmentation,  etc.
    
    

    \vspace{0.2cm}
    \textbf{Amount:} 1 - 3 pages
}

4 - Methods
\todo[inline, color=lightgray!40]
{
    Provide a detailed explanation of the machine learning algorithm(s) you will apply to your problems. In this project, you are allowed to use third-party implementations in your source code, but only if you can demonstrate that you understand how they work. This entails that you should include a proper explanation of your method(s), their training objective and how it is optimized, hyperparameters, strengths and weaknesses, and of course, why you chose them for your problem.

    \vspace{0.2cm}
    \textbf{Amount:} 2 - 4 pages 
}

5 - Results

\todo[inline, color=lightgray!40]
{
    Document the experiments you've run and discuss their outcomes. This includes not only results for the main inference task, but also instrumental objectives such as determining hyperparameters. Make sure that you explain how and why you evaluate your experiments the way you do (metrics, baselines etc.) and present your results with tables and figures wherever appropriate. 
    
    \vspace{0.2cm}
    Please ensure that all tables/figures you produce have descriptive x- and y-axis. Also, if you have more than one attribute shown, include a legend or describe it in the figure caption.
    Further, all tables included in the main part need to be described.
    
    \vspace{0.2cm}
    It might also be reasonable to split up this section. For instance, it could be more natural to first present the experiments and results in a purely objective way, and then add another section with your own subjective interpretation and discussion. 
    
    \vspace{0.2cm}
    Finally, don't be (too) disheartened by negative results. Honestly disclose the outcome of your experiments and analyze them to the best of your ability. If something didn't work out the way you thought, try to figure out why. Based on how much time there is left, you can either try to implement or describe possible solutions.
    
    \vspace{0.2cm}
    \textbf{Amount:} 2 - 4 pages
}

6 - Conclusion

\todo[inline, color=lightgray!40]
{
    Summarize your report, focusing on key findings and results. Why do you think you got the results that you got, what went well, and what could have been done better? Did the experiments reveal something interesting that might warrant further research? What would you have done if you had access to more data, compute, manpower, or time?
    
    \vspace{0.2cm}
    \textbf{Amount:} 0.5 - 1 page
}
